Addressing Graph Heterogeneity and Heterophily from A Spectral Perspective

Graph neural networks (GNNs) have demonstrated excellent performance in semi-supervised node classification tasks. Despite this, two primary challenges persist: heterogeneity and heterophily. Each of these two challenges can significantly hinder the performance of GNNs. Heterogeneity refers to a graph with multiple types of nodes or edges, while heterophily refers to the fact that connected nodes are more likely to have dissimilar attributes or labels. Although there have been few works studying heterogeneous heterophilic graphs, they either only consider the heterophily of specific meta-paths and lack expressiveness, or have high expressiveness but fail to exploit high-order neighbors. In this paper, we propose a Heterogeneous Heterophilic Spectral Graph Neural Network (H2SGNN), which employs two modules: local independent filtering and global hybrid filtering. Local independent filtering adaptively learns node representations under different homophily, while global hybrid filtering exploits high-order neighbors to learn more possible meta-paths. Extensive experiments are conducted on four datasets to validate the effectiveness of the proposed H2SGNN, which achieves superior performance with fewer parameters and memory consumption. The code is available at the GitHub repo: https://github.com/Lukangkang123/H2SGNN/.

==> 1_intro1.tex <==

\section{Introduction}
The past decade has witnessed the great success and prosperity of graph neural networks (GNNs) in diverse data science and engineering scenarios, such as traffic network \cite{traffic_network_1,traffic_network_2}, abnormal detection \cite{BWGNN,tang2024gadbench}, relational databases \cite{relational_databases_1,relational_databases_2} and recommender systems \cite{graph_recommendation1,graph_recommendation2}. 
Throughout the technical development, GNNs have been confronted with two persistent challenges: heterogeneity and heterophily. Each of these two challenges can significantly impede the performance of GNNs\cite{H2GB} Specifically, \textbf{heterogeneity} indicates multiple types of nodes or edges in a graph, which is called a \textit{heterogeneous} graph, while \textit{homogeneous} graph only has one type of node and edge. In contrast, \textbf{heterophily} characterizes a graph that how likely its connected nodes are different from each other \wrt the nodes' attributes or labels, where \textit{heterophilic} describes higher heterophily (\aka connected nodes have different labels) while \textit{homophilc} indicates lower heterophily (\aka connected nodes have similar labels). Based on these two characterizing perspectives of heterogeneity and heterophily, all the graphs can be sorted into four types: 1) homogeneous homophilic graph, 2) homogeneous heterophilic graph, 3) heterogeneous homophilic graph, and 4) heterogeneous heterophilic graph. As an example scenario of paper citation graph where the target nodes are papers, and the edges are the citation, writing, and publication relationships, we illustrate these four types of graphs in Figure~\ref{fig:demo}. 
\begin{figure}[t]   
	\centering 
	\includegraphics[width=\linewidth]{images/demo_new.pdf}
	\caption{Example of four types of graphs based on heterogeneity and heterophily. The horizontal axis is heterogeneity, which is divided into homogeneous and heterogeneous graphs from left to right. The vertical axis is heterophily, which is divided into homophilic and heterophilic graphs from bottom to top. "Paper" is the target node to be classified.}
 % \vspace{-4mm}
  \label{fig:demo}
\end{figure}





% In recent years, graph neural networks (GNNs) have garnered significant scholarly attention for their powerful capabilities in the data engineering community, such as traffic network\cite{traffic_network_1,traffic_network_2}, abnormal detection \cite{gaoaddressing,tang2024gadbench}, relational databases\cite{relational_databases_1,relational_databases_2,relational_databases_3} and recommender systems \cite{graph_recommendation1,graph_recommendation2}. Along with the entire research journey and development, GNNs have been confronted with two persistent challenges: heterogeneity and heterophily. Specifically, \textbf{Heterogeneity} indicates the degree of diversity regarding the node and edge types in a graph, where \textit{Heterogeneous} implies higher heterogeneity while \textit{Homogeneous} represents lower heterogeneity. In contrast, \textbf{Heterophily} characterizes a graph that how likely its connected nodes are differ with each other \wrt the nodes' attributes or labels, where \textit{Heterophilic} describes higher heterophily (\aka, connected nodes have similar labels) while \textit{Homophilc} indicates lower heterophily (\aka connected nodes have different labels). Based on these two characterizing perspectives of heterogeneity and heterophily, all the graphs can be sorted into four types: 1) Homogeneous Homophilc Graph, 2) Homogeneous Heterophilic Graph, 3) Heterogeneous Homophilic Graph, and 4) Heterogeneous Heterophilic Graph. As an example scenario of paper citation graph, where nodes are papers and edges are the citation relations among papers, we illustrate these four types of graphs in Figure~\ref{fig:demo}. 

% HDHGR \cite{HDHGR} notices the heterophily in heterogeneous graphs and

Among these four types of graphs, heterogeneous heterophilic graph exhibits the highest challenge while receiving the least research attention, despite their ubiquity in the real world. Concretely, most existing works focus either on heterophily in homogeneous graphs while overlooking the diversity of node and relation types~\cite{FAGCN,GPR-GNN,Mixhop,Geom-gcn}, or on heterogeneous GNNs based on the homophily assumption but neglecting heterophily in heterogeneous graphs~\cite{HAN,magnn,RGCN,mhgcn}. On the contrary, only a few attempts have been made to study the heterogeneous heterophilic Graph. Specifically, HDHGR \cite{HDHGR} notices degenerated performance when handling heterogeneous graphs with heterophily, and proposes a homophily-oriented deep heterogeneous graph rewiring method. Meanwhile, Hetero2Net \cite{Hetero2Net} proposes a heterophily-aware heterogeneous GNN that incorporates both masked meta-path prediction and masked label prediction tasks to handle heterophilic heterogeneous graphs. Even though some progress has been made, research on heterogeneous heterophilic graphs is still in its nascent stages, characterized by limited theoretical exploration and interoperability, as well as suboptimal performance.
Among these four types of graphs, heterogeneous heterophilic graph exhibits the highest challenge while receiving the least research attention, despite their ubiquity in the real world. Concretely, most existing works focus either on heterophily in homogeneous graphs while overlooking the diversity of node and relation types~\cite{FAGCN,GPR-GNN,Mixhop,Geom-gcn}, or on heterogeneous GNNs based on the homophily assumption but neglecting heterophily in heterogeneous graphs~\cite{HAN,magnn,RGCN,mhgcn}. On the contrary, only a few attempts have been made to study the heterogeneous heterophilic Graph. Specifically, HDHGR \cite{HDHGR} notices degenerated performance when handling heterogeneous graphs with heterophily, and proposes a homophily-oriented deep heterogeneous graph rewiring method. Meanwhile, Hetero2Net \cite{Hetero2Net} proposes a heterophily-aware heterogeneous GNN that incorporates both masked meta-path prediction and masked label prediction tasks to handle heterophilic heterogeneous graphs. Even though some progress has been made, research on heterogeneous heterophilic graphs is still in its nascent stages, characterized by limited theoretical exploration and interoperability, as well as suboptimal performance.

% \footnote{More related work can be found in Appendix G.}.

%To address these limitations, we seek to explore the potential of spectral GNNs, which have shown a solid theoretical foundation and remarkable interpretability~\cite{spectral_survey,benchmarking_Spectral,Spectralbenchmarking}. 
To address these limitations, spectral GNN demonstrates great potential in solving the heterophily and homogeity problems given its solid theoretical foundation and remarkable interpretability~\cite{spectral_survey,benchmarking_Spectral,Spectralbenchmarking}.
(1) In terms of heterophily~\cite{FAGCN,GPR-GNN,BernNet}, spectral GNNs typically learn adaptive filters that yield responses at varying frequencies, where a low-pass filter well captures the characteristic of homophilic graphs, while a high-pass filter caters the needs of heterophilic graphs.
%Spectral GNNs typically learn adaptive filters that yield responses at varying frequencies, where a low-pass filter is suitable for homophilic graphs, and a high-pass filter is suitable for heterophilic graphs. 
%As a result, spectral GNNs have been widely used to address heterophilic problems \cite{FAGCN,GPR-GNN,BernNet}.
(2) Regarding heterogeity, most of existing spectral GNN methods are only designed for homogeneous graphs~\cite{}, while significantly overlooking the scenarios of heterogeneous graphs. To the best of our knowledge, there is only one work, \aka, PSHGCN \cite{PSHGCN}, that applies spectral GNNs to heterogeneous graphs by leveraging multivariate polynomial filters (MPF). 
Despite the performance gain, MPF will induce exponential growth of parameters and memory, resulting in limitations when scaling up to large graphs in real world.
%However, spectral GNNs are typically designed on homogeneous graphs. Few works, such as PSHGCN \cite{PSHGCN}, attempt to apply spectral GNNs to heterogeneous graphs using multivariate polynomials as filters. 
%However, the exponential growth of parameters and memory with the order and the difficult-to-interpret filters limits its application. 
Therefore, this raises a question: \textit{Can spectral GNNs adaptively learn heterogeneous graphs under varying degrees of homophily, such as heterogeneous homophilic graphs and heterogeneous heterophilic graphs with low complexity and enhanced interpretability?} -- make it short.


                
% In recent years, GNNs have achieved excellent performance in graph learning tasks such as drug discovery \cite{drug_discovery3,drug_discovery4}, abnormal detection \cite{gaoaddressing,tang2024gadbench}, and recommendation systems \cite{graph_recommendation1,graph_recommendation2}.

% Nevertheless, GNNs still face two challenges: heterogeneity and heterophily. 
% x\textbf{Heterogeneity} describes a graph that contains multiple types of nodes or edges, whereas \textbf{heterophily} characterizes a graph where connected nodes are more likely to differ in their attributes or labels. Taking citation graphs as an example, where the goal is to predict the category of each paper, real-world graphs can be divided into the following four types:

% ysma rewritting: Along with the entire research journey and development, GNNs have been confronted with two persistent challenges: heterogeneity and heterophily. Specifically, \textbf{Heterogeneity} indicates the degree of diversity regarding the node and edge types in a graph, where \textit{Heterogeneous} implies higher heterogeneity while \textit{Homogeneous} represents lower heterogeneity. In contrast, \textbf{Heterophily} characterizes a graph that how likely its connected nodes are differ with each other \wrt the nodes' attributes or labels, where \textit{Heterophilic} describes higher heterophily (\aka, connected nodes have similar labels) while \textit{Homophilc} indicates lower heterophily (\aka connected nodes have different labels). Based on these two characterizing perspectives of heterogeneity and heterophily, all the graphs can be sorted into four types: 1) Homogeneous Homophilc Graph, 2) Homogeneous Heterophilic Graph, 3) Heterogeneous Homophilic Graph, and 4) Heterogeneous Heterophilic Graph. As an example scenario of paper citation graph, where nodes are papers and edges are the citation relations among papers, we illustrate these four types of graphs in Figure~\ref{fig:demo}. 

% \begin{itemize}

%  \item \textit{Homogeneous Homophilc Graph}: The connected nodes are similar to each other, and the node type and relation type are unique, as shown in Figure 1(a).
%  \item \textit{Homogeneous Heterophilic Graph}: The connected nodes may have different attributes or labels, but the node type and relation type are unique, as shown in Figure 1(b).
%  \item \textit{Heterogeneous Homophilic Graph}: The connected target nodes are similar to each other, but there are multiple nodes or relation types, as shown in Figure 1(c).
%  \item \textit{Heterogeneous Heterophilic Graph}: The connected target nodes may have different attributes or labels, and there are multiple nodes or relation types, as shown in Figure 1(d).
% \end{itemize}

% \begin{itemize}
%     \item \textit{Homogeneous Homophilic Graphs}: There is only one type of node and edge, and the connected nodes are similar. As depicted in Fig. 1(a), papers in the same category cite each other.
%     \item \textit{Homogeneous Heterophilic Graphs}: There is only one type of node and edge, but connected nodes may differ in attributes or labels. As illustrated in Fig. 1(b), papers in different categories cite each other.
%     \item \textit{Heterogeneous Homophilic Graphs}: There are multiple node and edge types, but the target nodes connected by meta-paths are similar. As shown in Fig. 1(c), an author or conference publishes papers in the same category.
%     \item \textit{Heterogeneous Heterophilic Graphs}: There are multiple node and edge types, and the target nodes connected by meta-paths may differ in attributes or labels, As presented in Fig. 1(d), an author or conference publishes papers in different categories.

% \end{itemize}

% Homogeneous homophilic graphs are the most widely studied. Methods designed for this type of graph typically aggregate neighbor node features to make connected nodes similar\cite{GCN,GAT,GraphSAGE}. For homogeneous heterophilic graphs, various approaches have been developed to address heterophily, including spectral GNNs \cite{FAGCN,GPR-GNN} and long-distance node exploration methods \cite{Mixhop}. For heterogeneous homophilic graphs, strategies to manage heterogeneity include meta-path-based methods \cite{HAN,magnn} and direct aggregation of diverse node types \cite{RGCN,mhgcn}.

%\textbf{Heterogeneity} describes a graph that contains multiple types of nodes or edges, whereas \textbf{heterophily} characterizes a graph where connected nodes are more likely to differ in their attributes or labels. Taking citation graphs as an example, where the goal is to predict the category of each paper, real-world graphs can be divided into the following four types:

% ysma rewritting: Among these four types of graphs, Heterogeneous Heterophilic Graph exhibits the highest challenge while receives least research attention. Concretely, most of existing works focus either on heterophily in homogeneous graphs while overlooking the diversity of node and relation types~\cite{FAGCN,GPR-GNN,Mixhop,Geom-gcn}, or on heterogeneous GNNs based on the homophily assumption but neglecting heterophily in heterogeneous graphs~\cite{HAN,magnn,RGCN,mhgcn}. As contrary, only a few attempts have been made to study the Heterogeneous Heterophilic Graph. Concretely, HDHGR\cite{HDHGR} notices the heterophily in heterogeneous graphs and proposes a homophily-oriented deep heterogeneous graph rewiring method. Hetero2Net \cite{Hetero2Net} proposes a heterophily-aware heterogeneous GNN that incorporates both masked meta-path prediction and masked label prediction tasks to handle heterophilic heterogeneous graphs. Even though some progress has been achieved, research on Heterogeneous Heterophilic Graph is still in its nascent stages, characterized by limited theoretical exploration and interoperability, as well as suboptimal performance.

% ysma rewritting: To address these limitations, we seek to explore the potential of spectral GNNs, which have shown solid theoretical foundation and remarkable interpretability~\cite{spectral_survey,benchmarking_Spectral}. Spectral GNNs typically learn adaptive filters that yield response at varying frequencies. Specifically, a low-pass filter is suitable for homophilic graphs, a high-pass filter is suitable for heterophilic graphs. Consequently, they have been widely used to address heterophilic problems \cite{FAGCN,GPR-GNN,BernNet}. However, spectral GNNs are typically designed on homogeneous graphs for graph-based data engineering. This raises a question: \textit{Can spectral GNNs adaptively learn heterogeneous graphs with varying degrees of homophily, such as heterogeneous homophilic graphs and heterogeneous heterophilic graphs?}

% The first three types of graphs have been extensively studied\cite{GCN,GAT,GraphSAGE,FAGCN,GPR-GNN,Mixhop,Geom-gcn,HAN,magnn,RGCN,mhgcn}. For example, data engineers predominantly focus either on heterophily in homogeneous graphs while overlooking the diversity of node and relation types\cite{FAGCN,GPR-GNN,Mixhop,Geom-gcn}, or on heterogeneous GNNs based on the homophily assumption but neglecting heterophily in heterogeneous graphs\cite{HAN,magnn,RGCN,mhgcn}. Nevertheless, in real-world applications, connected target nodes in heterogeneous graphs may have different categories. For instance, in a movie graph, films featuring the same actor may belong to different genres. Such graphs exhibit both heterogeneity and heterophily, aspects that are often ignored in current studies.

% Although there are few works focusing on heterogeneous heterophilic graphs \cite{HDHGR,Hetero2Net}, there is still a lack of theoretical and interpretable methods.

% For heterogeneous heterophilic graphs, few works have made useful attempts. In particular, HDHGR\cite{HDHGR} notices the heterophily in heterogeneous graphs and proposes a homophily-oriented deep heterogeneous graph rewiring method. Hetero2Net \cite{Hetero2Net} proposes a heterophily-aware heterogeneous GNN that incorporates both masked meta-path prediction and masked label prediction tasks to handle heterophilic heterogeneous graphs. However, compared with spectral GNNs, the above methods lack theoretical guarantees and interoperability, resulting in suboptimal performance.

% Spectral GNNs offer remarkable interpretability and a solid theoretical foundation\cite{spectral_survey,benchmarking_Spectral}, capable of learning adaptive filter responses at varying frequencies. For instance, a low-pass filter is suitable for homophilic graphs,  a high-pass filter is suitable for heterophilic graphs. Consequently, they are extensively used to address heterophilic problems \cite{FAGCN,GPR-GNN,BernNet}. However, spectral GNNs are typically designed on homogeneous graphs for graph-based data engineering. This raises a question: \textit{Can spectral GNNs adaptively learn heterogeneous graphs with varying degrees of homophily, such as heterogeneous homophilic graphs and heterogeneous heterophilic graphs?}

% Spectral GNNs possess excellent interpretability and a strong theoretical foundation. They can learn filter responses at different frequencies, such as low-pass, high-pass, and band-pass. Therefore, they are widely used to solve heterophilic problems. For example, a low-pass filter is suitable for homophilic graphs. Currently, the application of spectral GNN is limited to homogeneous graphs. Therefore, a natural question arises: \textit{Can spectral GNN adaptively learn heterogeneous graphs with different homophilic degrees? e.g., heterogeneous homophilic graph and heterogeneous heterophilic graph.} 




Achieving this objective presents two technical challenges. First, heterogeneous graphs may comprise subgraph combinations with diverse homophily degrees. For example, for the ACM dataset shown in Table \ref{tab:homophily}, the subgraphs induced by the $PAP$ and $PCP$ metapaths are homophilic graphs, while the $PKP$ metapath subgraph is a heterophilic graph. Addressing combinations and interactions of subgraphs with different homophily degrees is a significant challenge. Second, It is well known that in heterogeneous graphs, diverse meta-paths can learn powerful node representations to improve performance \cite{gtn,HGAMLP,LMSPS}. Nevertheless, spectral GNNs can only filter a predefined relationship matrix. Therefore, how to utilize spectral GNNs to explore and learn more meta-paths in heterogeneous graphs is another challenge.
 
% Recently, PSHGCN\cite{PSHGCN} attempts to apply spectral GNN to heterogeneous graphs. However, the number of its terms grows exponentially with the order, which limits its application.

% To address these challenges, we propose a \textbf{H}eterogeneous \textbf{H}eterophilic \textbf{S}pectral \textbf{G}raph \textbf{N}eural \textbf{N}etwork, short as H$^2$SGNN. 

To address these challenges, we propose a heterogeneous heterophilic spectral graph neural network, short as H$^2$SGNN.
First, to handle the diverse homophily of different subgraphs in heterogeneous graphs, we introduce \textbf{local independent filtering}, which segments the heterogeneous graph into subgraphs based on different meta-paths. Then we perform local independent polynomial filtering on each subgraph. Thus, we can adaptively learn node representations catering to diverse degrees of homophily along with different meta-paths. Furthermore, independent polynomial filtering for each meta-path is beneficial to enhance interpretability, for example, the learned low-pass filter represents a homophilic meta-path subgraph. Second, to capture the interaction of different meta-paths and learn more meta-paths, we propose \textbf{global hybrid filtering}. It measures and aggregates multiple meta-path matrices into a global adjacency matrix, on which we execute polynomial filtering operations. In addition, theoretical analysis demonstrates that the proposed global hybrid filtering is equivalent to a multivariate polynomial with enhanced expressiveness under certain conditions, with lower parameters and memory consumption. \textbf{Our contributions are summarized as follows:} 

% To our knowledge, this is the first attempt to apply spectral graph filters to heterogeneous heterophilic graphs.


\begin{itemize}[leftmargin=0.5cm, itemindent=0cm]
    \item We propose H$^2$SGNN, a novel heterogeneous heterophilic spectral graph neural network tailored to address heterophily and heterogeneity. To our knowledge, this is the first attempt to apply spectral GNN to address heterophily and heterogeneity simultaneously.
    % \item The proposed H$^2$SGNN can adaptively learn node representations of diverse homophily of different subgraphs. In addition, theoretical analysis shows that H$^2$SGNN can capture the interactions between different meta-paths and explore more meta-paths.
    \item We provide theoretical analysis and show that the proposed global hybrid filter is conditionally equivalent to a multivariate polynomial with enhanced expressive power.
    \item The proposed H$^2$SGNN enhances the interpretability of spectral GNN in heterogeneous graphs, because the learned filters can reflect the homophily of the graph.
    
    % At the same time, if the homophily of a meta-path in the graph is known, a filter for this meta-path can be designed in advance.
    \item We conduct extensive experiments on four datasets to validate the effectiveness of the proposed H$^2$SGNN, which achieves superior performance with fewer parameters and memory consumption.
\end{itemize}


% \section{Introduction}
% In recent years, graph neural networks (GNNs) have demonstrated exceptional performance in various graph learning tasks, such as drug discovery \cite{drug_discovery1,drug_discovery2}, molecular property prediction \cite{Molecular_GNN1,Molecular_GNN2}, and recommendation systems \cite{GNN_recommendation1,GNN_recommendation2}.

% However, GNNs face significant challenges, particularly in addressing heterophily and heterogeneity within graphs. These challenges can be categorized into four distinct types of graphs:
% \begin{itemize}
%     \item \textit{Homogeneous Homophilic Graphs}: Nodes that are connected tend to be similar, with uniform node and relation types, as depicted in Figure 1(a).
%     \item \textit{Homogeneous Heterophilic Graphs}: Nodes that are connected may differ in attributes or labels, but the node and relation types remain uniform, as illustrated in Figure 1(b).
%     \item \textit{Heterogeneous Homophilic Graphs}: Connected nodes are similar, but multiple node or relation types are present, as shown in Figure 1(c).
%     \item \textit{Heterogeneous Heterophilic Graphs}: Connected nodes may differ in attributes or labels, with multiple node and relation types, as depicted in Figure 1(d).
% \end{itemize}

% While homogeneous homophilic graphs are the most prevalent, homogeneous heterophilic and heterogeneous homophilic graphs have also been extensively studied. For homogeneous heterophilic graphs, various approaches have been developed to address heterophily, including spectral GNNs \cite{FAGCN,GPR-GNN} and long-distance node exploration methods \cite{Mixhop,Geom-gcn}. For heterogeneous homophilic graphs, strategies to manage heterogeneity include meta-path-based methods \cite{HAN,magnn} and direct aggregation of diverse node types \cite{RGCN,mhgcn}.

% Existing research predominantly focuses either on heterophily in homogeneous graphs, overlooking the diversity of node and relation types, or on heterogeneous GNNs based on the homophily assumption, neglecting potential heterophily in heterogeneous graphs. However, in real-world applications, connected nodes in heterogeneous graphs often exhibit dissimilarity. For instance, in a movie graph, films featuring the same actor may belong to different genres. Such graphs exhibit both heterogeneity and heterophily, aspects that are frequently ignored in current studies.

% Spectral GNNs offer remarkable interpretability and a robust theoretical foundation, capable of learning filter responses at varying frequencies (e.g., low-pass, high-pass, and band-pass). Consequently, they are extensively used to address heterophilic problems. For instance, a low-pass filter is suitable for homophilic graphs. However, the application of spectral GNNs is presently confined to homogeneous graphs. This raises a pertinent question: \textit{Can spectral GNNs adaptively learn heterogeneous graphs with varying degrees of homophily, such as heterogeneous homophilic and heterogeneous heterophilic graphs?}

% Achieving this objective presents several technical challenges. First, heterogeneous graphs encompass multiple node and relation types, necessitating modifications to typical spectral GNNs designed for homogeneous graphs. Second, heterogeneous graphs may comprise subgraph combinations with diverse homophily degrees. For example, a heterogeneous graph might include three homophilic subgraphs and one heterophilic subgraph. Addressing the interactions and combinations of subgraphs with different homophily degrees is another significant challenge.

% To address these challenges, we propose a \textbf{H}eterogeneous \textbf{S}pectral \textbf{G}raph \textbf{N}eural \textbf{N}etwork via graph filtering (H$^2$SGNN). Firstly, to manage the diverse node and relation types in heterogeneous graphs, we introduce local independent filtering. This method segments the heterogeneous graph into subgraphs based on different meta-paths corresponding to the target node type, and then applies independent polynomial filtering to each subgraph to learn node representations under various connection patterns. Secondly, to capture the interactions among different meta-paths, we aggregate multiple meta-paths into a global adjacency matrix, which is weighted appropriately, and perform polynomial filtering on this global matrix. This approach, termed global hybrid filtering, facilitates the learning of a broader range of meta-paths while optimizing resource consumption. Our contributions are summarized as follows:
% \begin{itemize}
%     \item We propose H$^2$SGNN, a novel heterogeneous spectral graph neural network designed to address the heterophily problem in heterogeneous graphs. To our knowledge, this is the first attempt to apply spectral graph filters to heterogeneous heterophilic graphs.
%     \item H$^2$SGNN integrates local independent filtering and global hybrid filtering. Local independent filtering aims to learn node representations of meta-paths under different connection patterns, while global hybrid filtering captures interactions between different meta-paths and explores additional meta-paths.
%     \item We conduct extensive experiments on four real-world datasets to validate the effectiveness of the proposed H$^2$SGNN. H$^2$SGNN achieves state-of-the-art performance with reduced parameters and memory requirements.
% \end{itemize}

\begin{table*}[t]
 \centering
 \caption{The homophily of different meta-path subgraphs on four datasets.}
% \begin{tabular}{llll|lll|lll|ll}
\begin{tabular}{cccc|ccc|ccc|cc}
\toprule
dataset   & \multicolumn{3}{c|}{ACM}           & \multicolumn{3}{c|}{DBLP} & \multicolumn{3}{c|}{IMDB} & \multicolumn{2}{c}{AMiner}\\
\midrule
meta-path &  PAP   & PCP   & PKP   & APA    & APTPA  & APVPA  & MDM    & MAM    & MKM    & PAP         & PRP        \\
% \midrule
homophily (\%) & 81.45 & 64.03 & 33.38 & 87.22 & 32.49 & 67.00 & 40.44 & 17.26 & 13.39 & 97.16   & 86.80 \\
\bottomrule
\label{tab:homophily}
\end{tabular}
\end{table*}


% Spectral GNNs on heterogeneous graphs need to be further explored.




% \begin{table}[t]
% \centering
% \caption{Existing HGNNs that attempt to design the spectral heterogeneous graph convolution.}
% \vspace{-2mm}
% \begin{tabular}{@{}lll@{}}
% \toprule
% Method &filter \\ \midrule
% GTN    &$\mathbf{D}^{-1}\prod\nolimits_{k=0}^{K}\sum\nolimits_{r=0}^{R}\alpha_{r}^{(k)}\mathbf{A}_r$  \\
% EMRGNN  &$\sum\nolimits_{k=0}^{K}\alpha(1-\alpha)^k \left(\sum\nolimits_{r=1}^{R}\mu_r\Tilde{\mathbf{A}}_{r} \right)^k$ \\
% MHGCN   &$\left( 
% \sum\nolimits_{r=1}^{R}\beta_r\mathbf{A}_r \right)^{K}$   \\ 
% PSHGCN & 
% $g(\hat{\mathbf{A}}_1,\hat{\mathbf{A}}_2,\ldots,\hat{\mathbf{A}}_R)^{\top}g(\hat{\mathbf{A}}_1,\hat{\mathbf{A}}_2,\ldots,\hat{\mathbf{A}}_R)$ \\
% ours &  $\left( 
% \sum\nolimits_{r=1}^{R}\beta_r\mathbf{A}_r \right)^{K}$  \\
% \bottomrule
% \end{tabular}
% \label{tb:hgnn_with_filter}
% \vspace{-2mm}
% \end{table}



==> 5_related.tex <==
% Existing GNNs can be divided into two categories: \emph{spatial GNNs} and \emph{spectral GNNs}. Spatial GNNs often adopt a message-passing mechanism to learn node representations by aggregating neighbor node features. In contrast,
\section{Related Work}
This section introduces related research, including spectral graph neural networks, heterogeneous homophilic GNNs, and heterogeneous heterophilic GNNs.
\subsection{Spectral Graph Neural Network}
Different from spatial GNNs based on message-passing, spectral GNNs map node features to a new desired space by selectively attenuating or amplifying the Fourier coefficients \(\hat{\mathbf{x}} = \mathbf{U}^{\top} \mathbf{x}\) induced by the normalized Laplacian matrix.


According to whether the filter can be learned, the spectral GNNs can be divided into \emph{pre-defined filters} and \emph{learnable filters}. In the category of pre-defined filters, GCN \cite{GCN} uses a simplified first-order Chebyshev polynomial. APPNP \cite{PPNP} utilizes Personalized Page Rank to set the weight of the filter. GNN-LF/HF \cite{GNN_LF_HF} designs filter weights from the perspective of graph optimization functions. In the category of learnable filters. ChebNet \cite{Chebyshev} uses Chebyshev polynomials with learnable coefficients. GPR-GNN \cite{GPR-GNN} extends APPNP by directly parameterizing its weights. BernNet \cite{BernNet} uses Bernstein polynomials to learn filters and forces all coefficients positive. JacobiConv \cite{JacobiConv} adopts an orthogonal and flexible Jacobi basis to accommodate a wide range of weight functions. ChebNetII\cite{ChebNetII} uses Chebyshev interpolation to learn filters. Specformer\cite{Specformer} performs self-attention in the spectral domain to learn a set-to-set spectral filter. FavardGNN\cite{OptBasisGNN} learns a polynomial basis from possible orthonormal bases.


% Recently, some works have applied spectral GNNs to node-level filtering. For example, DSF\cite{DSF} proposes a novel diversified spectral filtering framework that automatically learns node-specific filter weights to exploit the varying local structures. 


% By estimating the node-oriented spectral filter for each node. 
% NFGNN\cite{NFGNN} is provided with the capability of precise local node positioning via the generalized translated operator, thus discriminating the variations of local homophily patterns adaptively. 

% However, all these methods are designed for homogeneous graphs, and spectral GNNs on heterogeneous graphs need to be further explored.

Some work has explored spectral GNNs on multigraphs  or heterogeneous graphs. For example, MGNN \cite{MGNN} develops convolutional information processing on multigraphs and introduces convolutional multigraph neural networks. PSHGCN \cite{PSHGCN} proposes positive non-commutative polynomials to design positive spectral non-commutative graph convolution based on a unified graph optimization framework. However, the exponential growth of parameters and memory limits its application. Moreover, the multivariate polynomials are difficult to explain complex and diverse graph filters, such as low-pass, high-pass, band-pass, etc. 

\subsection{Heterogeneous Homophilic GNNs}
According to the way of processing different semantics, Heterogeneous Graph Neural Networks (HGNNs) can be broadly categorized into meta-path-based and meta-path-free methods. Meta-path-based methods use pre-defined meta-paths to propagate and aggregate neighbor features. For example, HAN \cite{HAN} leverages hierarchical attention to describe node-level and semantic-level structures. MAGNN \cite{magnn} improves HAN by introducing meta-path-based aggregation to learn semantic messages from multiple meta-paths. SeHGNN~\cite{sehgnn} employs pre-defined meta-paths for neighbor aggregation and incorporates a transformer-based method. 
 

Meta-path-free methods extend message passing and aggregation of GNNs to heterogeneous graphs without manually designed meta-paths. For example, RGCN~\cite{RGCN} extends GCN~\cite{GCN} by applying edge type-specific graph convolutions to heterogeneous graphs. GTN~\cite{gtn} employs soft sub-graph selection and matrix multiplication to create neighbor graphs. SimpleHGN~\cite{hgb} incorporates a multi-layer GAT network, utilizing attention based on node features and learnable edge-type embeddings. MHGCN~\cite{mhgcn} learns summation weights directly and uses GCN's convolution for feature aggregation. EMRGNN~\cite{emrgnn} and HALO~\cite{halo} propose optimization objectives for heterogeneous graphs and design their architectures by addressing these optimization problems. HINormer~\cite{hinormer} combines a local structure encoder and a relation encoder, using a graph Transformer to learn node embeddings. HGAMLP\cite{HGAMLP} uses a local multi-knowledge extractor and exploits a de-redundancy mechanism to extract pure graph structure information from high-order meta-paths.
However, none of these methods consider the heterophily in heterogeneous graphs.


\subsection{Heterogeneous Heterophilic GNNs}
HDHGR \cite{HDHGR} notices the heterophily phenomenon in heterogeneous graphs, and proposes a homophily-oriented deep heterogeneous graph rewiring method. Hetero2Net \cite{Hetero2Net} proposes a heterophily-aware heterogeneous GNN that incorporates both masked meta-path prediction and masked label prediction tasks to handle heterophilic heterogeneous graphs. SLHRec\cite{SLHRec} takes into account the heterogeneity in heterogeneous information networks and proposes a novel structure- and logic-aware heterogeneous graph learning framework for recommender systems. HERO \cite{HERO} proposed to learn a self-expressive matrix to capture homogeneity from subspaces and nearby neighbors for self-supervised heterogeneous graph learning. However, compared with spectral GNNs, the above methods have limited theoretical exploration and interpretability, resulting in suboptimal performance.



